Taming mismatches in inter-agent distances for the formation-motion control of second-order agents

This paper presents the analysis on the influence of distance mismatches on the standard gradient-based rigid formation control for second-order agents. It is shown that, similar to the first-order case as recently discussed in the literature, these mismatches introduce two undesired group behaviors: a distorted final shape and a steady-state motion of the group formation. We show that such undesired behaviors can be eliminated by combining the standard formation control law with distributed estimators. Finally, we show how the mismatches can be effectively employed as design parameters in order to control a combined translational and rotational motion of the formation.

==> FIGsquare.tex <==
% Sketch output, version 0.3 (build 7d, Sun Mar 20 14:11:05 2016)
% Output language: PGF/TikZ,LaTeX
\begin{tikzpicture}[line join=round]
\draw(0,0)--(1,0)--(1,1)--(0,1)--(0,0);
\filldraw(0,0) circle (2pt);
\filldraw(1,0) circle (2pt);
\filldraw(1,1) circle (2pt);
\filldraw(0,1) circle (2pt);
\end{tikzpicture}% End sketch output


==> Makefile <==
all: motion_di.pdf Art40HectorJayawardhanaCao.pdf

clean:
	$(RM) *~ *.pdf *.dvi *.log *.aux *.bbl *.blg *.toc *.lol *.loa *.lox \
		*.lot *.out *.lg *.tmp *.xref *.lof .*.swp

motion_di.pdf: motion_di.tex
	sketch FIGsquare.sk -o FIGsquare.tex
	sketch FIGsquaredef.sk -o FIGsquaredef.tex
	sketch FIGsquareRig.sk -o FIGsquareRig.tex
	sketch FIGtetra.sk -o FIGtetra.tex
	pdflatex motion_di
	bibtex motion_di
	pdflatex motion_di
	pdflatex motion_di

Art40HectorJayawardhanaCao.pdf: Art40HectorJayawardhanaCao.tex
#	sketch FIGsquare.sk -o FIGsquare.tex
#	sketch FIGsquaredef.sk -o FIGsquaredef.tex
#	sketch FIGsquareRig.sk -o FIGsquareRig.tex
#	sketch FIGtetra.sk -o FIGtetra.tex
	pdflatex Art40HectorJayawardhanaCao
	bibtex Art40HectorJayawardhanaCao
	pdflatex Art40HectorJayawardhanaCao
	pdflatex Art40HectorJayawardhanaCao

